Revisiting Path Contraction and Cycle Contraction

The Path Contraction and Cycle Contraction problems take as input an undirected graph $G$ with $n$ vertices, $m$ edges and an integer $k$ and determine whether one can obtain a path or a cycle, respectively, by performing at most $k$ edge contractions in $G$. We revisit these NP-complete problems and prove the following results. Path Contraction admits an algorithm running in $\mathcal{O}^*(2^{k})$ time. This improves over the current algorithm known for the problem [Algorithmica 2014]. Cycle Contraction admits an algorithm running in $\mathcal{O}^*((2 + \epsilon_{\ell})^k)$ time where $0 < \epsilon_{\ell} \leq 0.5509$ is inversely proportional to $\ell = n - k$. Central to these results is an algorithm for a general variant of Path Contraction, namely, Path Contraction With Constrained Ends. We also give an $\mathcal{O}^*(2.5191^n)$-time algorithm to solve the optimization version of Cycle Contraction. Next, we turn our attention to restricted graph classes and show the following results. Path Contraction on planar graphs admits a polynomial-time algorithm. Path Contraction on chordal graphs does not admit an algorithm running in time $\mathcal{O}(n^{2-\epsilon} \cdot 2^{o(tw)})$ for any $\epsilon > 0$, unless the Orthogonal Vectors Conjecture fails. Here, $tw$ is the treewidth of the input graph. The second result complements the $\mathcal{O}(nm)$-time, i.e., $\mathcal{O}(n^2 \cdot tw)$-time, algorithm known for the problem [Discret. Appl. Math. 2014].

==> intro-long.tex <==
% !TEX root = ./main.tex
Graph editing problems have consistently been benchmark problems against which the power of new algorithmic tools and techniques are tested. %a central role in the area of graph algorithms by providing
Typical editing operations are vertex deletions, edge deletions, edge additions, edge subdivisions and edge contractions. In this work, we focus on editing a simple undirected graph by only performing edge contractions. Contracting an edge results in the addition of a new vertex adjacent to the neighbors of its endpoints followed by the deletion of the endpoints. One may view an edge contraction as ``merging'' its endpoints into one thereby making them indistinguishable. Any loops or parallel edges created in the process are deleted so that the graph remains simple. In graph contraction problems, given a graph $G$ and an integer $k$, the interest is in determining if $G$ can be modified into a graph that belongs to a specific family of graphs by a sequence of at most $k$ edge contractions. Most basic such graph families are paths and cycles. This brings us to the problems studied in this paper, namely, \textsc{Path Contraction} and \textsc{Cycle Contraction}. 

In \textsc{Path Contraction} and \textsc{Cycle Contraction}, the objective is to determine if a path or a cycle respectively can be obtained from the input undirected graph $G$ on $n$ vertices by a sequence of at most $k$ edge contractions. 

\defproblem{\textsc{Path Contraction}}{A connected undirected graph $G$ and an integer $k$.}{Can one contract at most $k$ edges in $G$ to obtain a path?}

\defproblem{\textsc{Cycle Contraction}}{A connected undirected graph $G$ and an integer $k$.}{Can one contract at most $k$ edges in $G$ to obtain a cycle?}

\noindent Let $P_{\ell}$ and $C_{\ell}$ denote the path and cycle respectively on $\ell$ vertices. When viewed as vertex sets rather than graphs, $P_{\ell}$ and $C_{\ell}$ are referred to as induced $\ell$-path and induced $\ell$-cycle, respectively. Early results by Brouwer and Veldman~\cite{BrouwerV87} show that \textsc{Path Contraction} and \textsc{Cycle Contraction} are \NP-complete\ even when the target graph (which is a path or a cycle) has four vertices (i.e., when $k=n-4$). However, \textsc{Path Contraction} and \textsc{Cycle Contraction} are polynomial-time solvable when the target graph is a $P_{3}$ or a $C_{3}$~\cite{BrouwerV87}. In fact, Brouwer and Veldman~\cite{BrouwerV87} showed that \textsc{Path Contraction} is \NP-complete\  when the target path has $\ell$ vertices for every $\ell \ge 4$. Later, Hammack~\cite{Hammack02} showed that \textsc{Cycle Contraction} is \NP-complete\ when the target cycle has $\ell$ vertices for every $\ell \ge 5$. These results imply that \textsc{Path Contraction} and \textsc{Cycle Contraction} are \NP-complete\ in general. 

\textsc{Path Contraction} is one of the first graph contraction problems to be studied in the parameterized complexity framework. The most natural parameter is $k$ and Heggernes et al.~\cite{HeggernesHLLP14} showed that \textsc{Path Contraction} admits a kernel with at most $5k+3$ vertices and an \FPT\ algorithm running in $\calO^*(2^{k + o(k)})$ time. They also showed that \textsc{Path Contraction} can be solved in $\mathcal{O}^*(2^n)$ time by a simple algorithm -- color the graph with two colors, contract the connected components in the monochromatic subgraphs and check if the resulting graph is a path. Later, Li et al.~\cite{LI201720} improved the size of the kernel to at most $3k+4$ vertices. While there is no improvement to the $\calO^*(2^{k + o(k)})$-time algorithm known till date, Agrawal et al.~\cite{AgrawalFLST20} gave an $\mathcal{O}^*(1.99987^n)$-time algorithm  breaking the $\mathcal{O}^*(2^n)$ barrier. 

Our approach to \textsc{Path Contraction} has a different style when compared to these results. We focus on the following variant of \textsc{Path Contraction}. 

\defproblem{\textsc{Path Contraction With Constrained Ends}}{A connected undirected graph $G$, two disjoint subsets $X,Y \subseteq V(G)$ and an integer $k$.}{Can one contract at most $k$ edges in $G$ to obtain a $x^*$-$y^*$-path such that all vertices in $X$ are merged into $x^*$ and all vertices in $Y$ are merged into $y^*$?}.

\noindent Our first result is an algorithm for this problem using a dynamic programming formulation that crucially uses the notions of \textit{potential $k$-witness sets} (Definition \ref{def:k-potential-witness-set}) and \textit{potential $k$-prefix sets} (Definition \ref{def:k-nice-subset}). It is inspired by the exact exponential-time algorithm by Agrawal et al.~\cite{AgrawalFLST20} for \textsc{Path Contraction} and an \FPT\ algorithm by Saurabh et al.~\cite{SaurabhST20} for \textsc{Grid Contraction}. 

%\begin{itemize}
%    \item (Theorem~\ref{thm:path-ends-fpt-algo}) \textsc{Path Contraction With Constrained Ends} can be solved in $\mathcal{O}^*(2^{k-|X|-|Y|})$ time. 
%\end{itemize}
\begin{restatable}[]{thm}{pathEndsfptalgo}
\label{thm:path-ends-fpt-algo}
\textsc{Path Contraction With Constrained Ends} admits an algorithm
running in time $\mathcal{O}^*(2^{k-|X|-|Y|})$.
\end{restatable}


\noindent Observe that \textsc{Path Contraction With Constrained Ends} when $X=\emptyset$ and $Y=\emptyset$ is \textsc{Path Contraction}. Therefore, we obtain an algorithm for \textsc{Path Contraction}.

%\begin{itemize}
%    \item (Theorem~\ref{thm:path-fpt-algo}) \textsc{Path Contraction} can be solved in $\mathcal{O}^*(2^{k})$ time. 
%\end{itemize}

\begin{corollary}
\label{cor:path-conn-algo}
\textsc{Path Contraction} admits an algorithm
running in time $\mathcal{O}^*(2^{k})$.
\end{corollary}

%Our first result is an algorithm for \textsc{Path Contraction} with $\mathcal{O}^*(2^k)$ running time (Theorem~\ref{thm:path-fpt-algo}) . We show this result by giving an algorithm to solve the following Our algorithm for \textsc{Path Contraction With Constrained Ends} runs in $\mathcal{O}^*(2^{k-|X|-|Y|})$ time (Theorem~\ref{thm:path-ends-fpt-algo}) leading to an $\mathcal{O}^*(2^k)$-time algorithm for \textsc{Path Contraction}. The algorithm is a dynamic programming algorithm that uses ideas entirely different from that of the algorithm by Heggernes et al.~\cite{HeggernesHLLP14} and crucially uses the notions of \textit{potential $k$-witness sets} (Definition \ref{def:k-pot-pen-wit-set} and Definition \ref{def:k-pot-int-wit-set}) and \textit{potential $k$-prefix sets} (Definition \ref{def:k-nice-subset}). 

\noindent This is the first improvement for \textsc{Path Contraction} since its fixed-parameter tractability was established by Heggernes et al.~\cite{HeggernesHLLP14}. 

Our original motivation for focusing on \textsc{Path Contraction With Constrained Ends} was to understand its applicability in designing faster algorithms for \textsc{Cycle Contraction} since deleting one vertex from a cycle results in a path whose endpoints are neighbours of the deleted vertex. As cycles have treewidth $2$, one may use Courcelle’s theorem to show the existence of \FPT\ algorithms for \textsc{Cycle Contraction} (see \cite[Chapter 7]{CyganFKLMPPS15} for related definitions and arguments). However, the resulting algorithm has huge exponential factors in the running time. Belmonte et al.~\cite{BelmonteGHP14} showed that \textsc{Cycle Contraction} admits a kernel with at most $6k+6$ vertices which was later improved to $5k+4$ by Sheng and Sun~\cite{SHENG201914}. This immediately results in a single-exponential time algorithm, i.e., an $\mathcal{O}^*(c^k)$-time algorithm for some constant $c>200$, for \textsc{Cycle Contraction} -- simply color the graph with two or three colors, contract the connected components in the monochromatic subgraphs and check if the resultant graph is a cycle. We describe a faster algorithm using the algorithm for \textsc{Path Contraction With Constrained Ends} as a subroutine. 

%\begin{itemize}
%    \item (Theorem~\ref{thm:fpt-algo-cycle}) \textsc{Cycle Contraction} can be solved in $\mathcal{O}^*(2 + \epsilon_{\ell})^k$ where $0 < \epsilon_{\ell}  \leq  0.5509$ and $\epsilon_\ell$ is inversely proportional to $\ell = n - k$. 
%\end{itemize}
\begin{restatable}[]{thm}{fptalgocycle}
\label{thm:fpt-algo-cycle}
\textsc{Cycle Contraction} admits an algorithm running in time
$\mathcal{O}^*((2 + \epsilon_{\ell})^k)$ where 
$0 < \epsilon_{\ell}  \leq  0.5509$ and $\epsilon_\ell$ is inversely
proportional to $\ell = n - k$. 
\end{restatable}


\noindent This also implies an exact exponential-time algorithm for \textsc{Cycle Contraction} that runs in $\mathcal{O}^*(2.5509^n)$ time. We further improve the running time to $\mathcal{O}^*(2.5191^n)$ (Theorem \ref{thm:exact-algo-cycle}). 

%We show that \textsc{Cycle Contraction} can be solved in $\mathcal{O}^*(2.5508^k)$ time (Theorem~\ref{thm:fpt-algo-cycle}). %To our pleasant surprise, it turns out that \textsc{Path Contraction With Constrained Ends} is also useful in solving \textsc{Cycle Contraction}. \todo{K:add}

\textsc{Cycle Contraction} is related to an important graph parameter, namely, \textit{cyclicity}. The cyclicity of a graph is the largest integer $\ell$ such that the graph is contractible to $C_\ell$. This parameter was introduced by Blum~\cite{Blum82} and ever since there have been efforts towards understanding the complexity of computing cyclicity. The result of Brouwer and Veldman~\cite{BrouwerV87} which shows that \textsc{Cycle Contraction} is \NP-complete\ even when the target cycle is $C_4$ proves that computing cyclicity is \NP-hard\ in general. This result led to the study of the problem on special graph classes. Hammack~\cite{Hammack99} showed that the cyclicity of planar graphs can be computed in polynomial time. Therefore, \textsc{Cycle Contraction} is polynomial-time solvable on planar graphs. However, the status of \textsc{Path Contraction} on planar graphs is open. We resolve this question by showing the following result.

%\begin{itemize}
%    \item (Theorem~\ref{thm:path-planar}) \textsc{Path Contraction} on planar graphs is polynomial-time solvable.
%\end{itemize}

\begin{restatable}[]{thm}{pathplanar}
\label{thm:path-planar}
\textsc{Path Contraction} on planar graphs admits a polynomial-time
algorithm.
\end{restatable}

\noindent This result uses the \textsc{Cycle Contraction} algorithm on planar graphs as a subroutine to obtain a polynomial-time algorithm for \textsc{Path Contraction}. 

On chordal graphs, while \textsc{Cycle Contraction} is trivially solvable (in linear time), the status of \textsc{Path Contraction} is interesting. Heggernes et al.~\cite{HeggernesHLP14} proved that \textsc{Path Contraction} is polynomial-time solvable on chordal graphs by giving an $\mathcal{O}(nm)$-time algorithm where $m$ is the number of edges in the input graph. In fact, they showed a stronger result -- every connected chordal graph $G$ can be contracted to $P_{dia(G)+1}$ where $dia(G)$ denotes the diameter of $G$ (the maximum number of edges in a shortest path between two vertices). As no graph $G$ can be contracted to a path with more than $dia(G)+1$ vertices, this result is the best possible. As graphs with treewidth $tw$ are $tw$-degenerate\footnote[2]{A graph is $d$-degenerate if every non-empty subgraph has a vertex of degree at most $d$} and $tw$-degenerate graphs on $n$ vertices have at most $tw.n$ edges, it follows that any graph of treewidth $tw$ on $n$ vertices has at most $tw.n$ edges~\cite{CyganFKLMPPS15}. Hence, the $\mathcal{O}(nm)$-time algorithm for \textsc{Path Contraction} on chordal graphs is also an $\mathcal{O}(n^2 \cdot tw)$-time algorithm where $tw$ is the treewidth of $G$. %This algorithm is an $\mathcal{O}(n^2 \cdot tw)$-time algorithm where $tw$ is the treewidth of the input graph. 

Fine-grained complexity aims at making finer distinctions between problems based on their resource (like time, space) requirement. A crucial difference between the fine-grained complexity program and the theory of \NP-hardness is that all \NP-complete problems form an equivalence class -- if one of them is polynomial-time solvable, then all of them are. In contrast, there are few equivalence classes known in the realm of fine-grained complexity. One such class contains the \textsc{Orthogonal Vectors} problem. In the \textsc{Orthogonal Vectors} problem, given two sets of $n$ $d$-dimensional boolean vectors $X=\{x_1, x_2, \ldots, x_n\}$ and $Y=\{y_1, y_2, \ldots, y_n\}$, the objective is to determine if there is a pair of vectors $x_i \in X$ and $y_j \in Y$ that are orthogonal, i.e., $\langle x_i \cdot y_j \rangle= 0$. It is easy to see that \textsc{Orthogonal Vectors} can be solved in $\calO(n^2 d)$ time. The Orthogonal Vectors Conjecture~\cite{WilliamsY14} states that \textsc{Orthogonal Vectors} cannot be solved in $\calO(n^{2-\epsilon})$ time for any $\epsilon > 0$ when $d=\mathcal{O}(\log n)$. By giving a fine-grained reduction from \textsc{Orthogonal Vectors} to \textsc{Path Contraction} on split graphs (which is a subclass of chordal graphs), we show the following result.

%\begin{itemize}
%    \item (Theorem~\ref{thm:chordal-lb}) \textsc{Path Contraction} on chordal graphs cannot be solved in $\mathcal{O}(n^{2-\epsilon} \cdot 2^{o(tw)})$ time under the Orthogonal Vectors Conjecture.
%\end{itemize}

\begin{restatable}[]{thm}{chordallb}
\label{chordallb}
Unless the \textsf{Orthogonal Vectors Conjecture} fails,
\textsc{Path Contraction} on chordal graphs does not admit
an algorithm running in time 
$\mathcal{O}(n^{2-\epsilon} \cdot 2^{o(tw)})$
for any $\epsilon > 0$.
\end{restatable}

\noindent This result specifically shows that the $\mathcal{O}(n^2 \cdot tw)$-time algorithm given by Heggernes et al. is optimal -- if one wishes to reduce the quadratic dependency on $n$, an exponential overhead in terms of treewidth is inevitable. 

%We also give an algorithm for the problem that runs in $\mathcal{O}(n \cdot tw \cdot 2^{tw})$ time. 

%breaking 3^n for cycle is easy?
%cycle kernel Our result showcases how to design kernelization algorithm for one problem by exploiting kernels of another problem.
%As the \textsc{Path Contraction} problem admits a kernel with at most $5k + 3$ vertices~\cite[Theorem ~$6$]{HeggernesHLP14} (also see [Theorem 4.4] ~\cite{LI201720} for a kernel with at most $3k + 4$ vertices), it is sufficient to present an algorithm running in time $\calO(2^k \cdot n^{2})$.
%In the \FPT\ algorithm for \textsc{Cycle Contraction} we make use of some of structural aspects of contracting a graph to Cycle and then use the \FPT\ algorithm for \textsc{Path Contraction with Constrained Ends} as subroutine.
